Models and Benchmarks for Representation Learning of Partially Observed Subgraphs

Subgraphs are rich substructures in graphs, and their nodes and edges can be partially observed in real-world tasks. Under partial observation, existing node- or subgraph-level message-passing produces suboptimal representations. In this paper, we formulate a novel task of learning representations of partially observed subgraphs. To solve this problem, we propose Partial Subgraph InfoMax (PSI) framework and generalize existing InfoMax models, including DGI, InfoGraph, MVGRL, and GraphCL, into our framework. These models maximize the mutual information between the partial subgraph's summary and various substructures from nodes to full subgraphs. In addition, we suggest a novel two-stage model with $k$-hop PSI, which reconstructs the representation of the full subgraph and improves its expressiveness from different local-global structures. Under training and evaluation protocols designed for this problem, we conduct experiments on three real-world datasets and demonstrate that PSI models outperform baselines.

==> files/alg_model.tex <==

\begin{algorithm}
\caption{Partial Subgraph InfoMax framework}\label{alg:psi}
\KwData{The global graph $\gG = (\sV^{\glob}, \sA^{\glob}), \mX^{\glob}$ and a partially observed subgraph $\gS^{\obs}$ in $\sS^{\obs}$: $\gS^{\obs} = (\sV^{\obs}, \sA^{\obs}), \vg, \mX^{\obs} = \mX^{\glob}[\sV^{\obs}]$}
\KwResult{A logit vector of $\gS^{\obs}$: $\vy \in \sR^{C}$.}

1. Encode nodes in the partial subgraph: $\mH^{\obs} = \gE ( \mX^{\obs}, \sA^{\obs} )$.

2. Create the partial subgraph summary: $\vs^{\obs} = \gR (\mH^{\obs})$.

3. Compute a logit vector: $\vy = \gF (\vs^{\obs}, [\vg])$. We also use a subgraph-level feature $\vg$ in the final prediction if exists.

4. In the training stage, optimize losses to update parameters:

\If{training}
{
    a. Draw negative subgraph(s): $\gS^{-} = (\sV^{-}, \sA^{-}) \in \sS$.
    
    b. Augment full and negative subgraphs if necessary:
    
    \If{graph augmentations are used}{
        $\gS^{\sub}, \gS^{-} = \textrm{Aug}(\gS^{\sub}), \textrm{Aug}(\gS^{-})$.
    }
    
    c. Encode nodes in full and negative subgraphs, then summarize them if necessary:
    $\mH^{\sub} = \gE ( \mX[\sV^{\sub}], \sA^{\sub} \ \textor\ \sA^{\glob}[\sV^{\sub}] ),$
    $\mH^{-} = \gE ( \mX[\sV^{-}], \sA^{-} \ \textor\ \sA^{\glob}[\sV^{-}] ),$
    
    \ \ $\vs^{\sub},\ \vs^{\ -} = \gR (\mH^{\sub}),\ \gR (\mH^{-})$.
    
    d. Compute $\gL^{\textrm{GD}\ \textor\ \textrm{InfoNCE}}$ with the partial subgraph summary ($\vs^{\obs}$), positive ($\mH^{\sub}$ or $\vs^{\sub}$) and negative ($\mH^{-}$ or $\vs^{\ -}$) samples (Equations~\ref{eq:infomax_loss} and \ref{eq:infonce_loss}).
    
    e. Compute the cross-entropy loss $\gL^{\textrm{graph}}$ on the logit $\vy$ and label $y$, and minimize $\gL^{\textrm{graph}} + \lambda \gL^{\textrm{GD}\ \textor\ \textrm{InfoNCE}}$.
}

\end{algorithm}

==> files/fig_model_k_hop_psi.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.445\textwidth]{figures/PSI_model_2.pdf}
  \vspace{-0.33cm}
  \caption{Overview of the $k$-hop PSI.}
  \vspace{-0.5cm}
  \label{fig:model_two_stage}
\end{figure}


==> files/fig_model_two_stage.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{figures/PSI_model_2.pdf}
  \vspace{-0.3cm}
  \caption{Overview of the two-stage PSI model. The reconstructed summary $\vs^{\khop}$ from $k$-hop PSI distinguishes positive and negative substructures in the second PSI model. Then, two InfoMax losses are jointly optimized.}
  \vspace{-0.25cm}
  \label{fig:model_two_stage}
\end{figure}


==> files/fig_observed_nodes_eval.tex <==

\begin{figure}[t]
  \centering
  \includegraphics[width=0.28\textwidth]{figures/fig_line_obs_eval_Dataset_Dataset.pdf}
  \caption{Performance by \# of observed nodes at the \textit{test}.}
  \label{fig:num_obs_eval}
\end{figure}

\cmt{

\begin{wrapfigure}{R}{0.29\textwidth}
    \vspace{-0.7cm}
    \begin{center}
    \includegraphics[width=0.28\textwidth]{figures/fig_line_obs_eval_Dataset_Dataset.pdf}
    \end{center}
    \vspace{-0.4cm}
    \caption{Performance by \# of observed nodes at the \textit{test}.}
    \label{fig:num_obs_eval}
    \vspace{-0.8cm}
\end{wrapfigure}

}

==> files/fig_observed_nodes_xx.tex <==
\begin{wrapfigure}{R}{0.29\textwidth}
    \vspace{-0.65cm}
    \begin{center}
    \includegraphics[width=0.28\textwidth]{figures/fig_line_obs_xx_Dataset_Dataset.pdf}
    \end{center}
    \vspace{-0.4cm}
    \caption{Performance by \# of observed nodes at \textit{test and training}. The shaded area is the standard deviation.}
    \label{fig:num_obs_xx}
    \vspace{-0.7cm}
\end{wrapfigure}


==> files/fig_problem.tex <==
\begin{figure*}[t]
  \centering
  \vspace{-0.17cm}
  \includegraphics[width=0.8\textwidth]{figures/PSI_problem.pdf}
  \vspace{-0.33cm}
  \caption{Left: Comparison of subgraph and partial subgraph representation learning. The latter learns subgraph representations with partial observation of nodes and edges. Middle \& Right: Real-world examples of partial subgraph learning: fake news early detection and disease diagnosis with partial observation. See \textit{Real-world examples} in \S\ref{paragraph:real-world-examples} for a more detailed description.}
  \label{fig:problem}
  \vspace{-0.34cm}
\end{figure*}


==> files/table_edge.tex <==
\begin{table}[]% \vspace{-0.15cm}
\centering
\caption{Performance of the $k$-hop PSI + PS-InfoGraph by edge types on the ordered dataset, \FNTN.}
\label{tab:edge_inclusion}
\vspace{-0.22cm}
\begin{tabular}{ll}
\hline
Edge type                 & \FNTN \\ \hline
$\sA^{\sub}$              & $88.2_{\pm 1.4}$     \\
$\sA^{\glob}[\sV^{\sub}]$ & $89.6_{\pm 1.8}$     \\ \hline
\end{tabular}
\vspace{-0.32cm}
\end{table}

==> files/table_main_result_2_col.tex <==

\begin{table*}[]
\centering
\caption{Mean and standard deviation of the classification accuracy of five runs. The first column represent the number of observed nodes $ | \sV^{\obs} | $ used in each experiment (See \S\ref{sec:experimental_set_up} for more details) and settings corresponding to datasets are indicated with daggers ($\dag, \ddag$). \colorbox{weakblue}{The PSI model that outperforms} \colorbox{weakred}{the best baseline} (except for \colorbox{weakgray}{the oracle}) is indicated by color, and statistically significance by unpaired \ttest\ is denoted by asterisks (\colorbox{midblue}{**$\text{\pvalue} < .001$, *$\text{\pvalue} < .1$}).}
\vspace{-0.1cm}
\label{tab:main_result}
\begin{tabularx}{0.8\textwidth}{llXXX}
\hline
The \# of observed nodes    & Model        & \FNTN$^{\ddag}$             & \EMUser$^{\ddag}$ & \HPOMetab$^{\dag}$   \\ \hline
100\%                 & GraphSAGE    & \cellwg$86.3_{\pm 0.7}$    &\cellwg$82.1_{\pm 1.2}$ &\cellwg$47.7_{\pm 3.3}$ \\ \hline
                      & MLP          & $82.5_{\pm 2.6}$           & $71.9_{\pm 4.6}$       & $43.5_{\pm 4.4}$       \\
                      & GCN          & $84.6_{\pm 2.0}$           &\cellwr$72.8_{\pm 3.8}$ & $42.9_{\pm 1.8}$       \\
                      & GraphSAGE    & $84.9_{\pm 1.3}$           & $68.1_{\pm 2.6}$       &\cellwr$44.1_{\pm 1.3}$ \\
                      & GAT          &\cellwr$85.1_{\pm 0.8}$     & $71.5_{\pm 5.7}$       & $43.1_{\pm 2.3}$       \\
                      & SubGNN       & N/A                        & $61.3_{\pm 5.4}$       & $37.1_{\pm 1.5}$       \\ \cline{2-5} 
                      & PS-DGI       &\cellmb$87.5_{\pm 1.2}^{*}$ & $72.3_{\pm 6.2}$       & $44.0_{\pm 1.8}$       \\
$8^{\ddag}, 4^{\dag}$ & PS-InfoGraph &\cellmb$87.3_{\pm 0.0}^{**}$&\cellwb$75.7_{\pm 3.9}$ &\cellmb$47.1_{\pm 2.1}^{*}$   \\
                      & PS-MVGRL     &\cellmb$88.6_{\pm 0.9}^{**}$& OOM                    &\cellwb$45.4_{\pm 2.4}$       \\
                      & PS-GraphCL   &\cellmb$88.1_{\pm 1.3}^{*}$ &\cellwb$75.3_{\pm 2.4}$ &\cellmb$47.2_{\pm 3.5}^{*}$   \\
                      & $k$-hop PSI  &\cellmb$87.8_{\pm 1.2}^{*}$ &\cellwb$75.3_{\pm 2.4}$ & $42.4_{\pm 2.6}$      \\ \cline{2-5} 
                      & $k$-hop PSI + PS-DGI  &\cellmb$88.0_{\pm 0.7}^{**}$ &\cellwb$75.7_{\pm 4.4}$     &  $43.6_{\pm 1.0}$  \\
                      & $k$-hop PSI + PS-InfoGraph &\cellmb$89.6_{\pm 1.8}^{**}$ &\cellmb$77.0_{\pm 5.2}^{*}$ &\cellwb$44.6_{\pm 1.6}$ \\ \hline
\end{tabularx}
\vspace{-0.0cm}
\end{table*}

